Functional Collection Programming with Semi-Ring Dictionaries

This paper introduces semi-ring dictionaries, a powerful class of compositional and purely functional collections that subsume other collection types such as sets, multisets, arrays, vectors, and matrices. We developed SDQL, a statically typed language that can express relational algebra with aggregations, linear algebra, and functional collections over data such as relations and matrices using semi-ring dictionaries. Furthermore, thanks to the algebraic structure behind these dictionaries, SDQL unifies a wide range of optimizations commonly used in databases (DB) and linear algebra (LA). As a result, SDQL enables efficient processing of hybrid DB and LA workloads, by putting together optimizations that are otherwise confined to either DB systems or LA frameworks. We show experimentally that a handful of DB and LA workloads can take advantage of the SDQL language and optimizations. SDQL can be competitive with or outperforms a host of systems that are state of the art in their own domain: in-memory DB systems Typer and Tectorwise for (flat, not nested) relational data; SciPy for LA workloads; sparse tensor compiler taco; the Trance nested relational engine; and the in-database machine learning engines LMFAO and Morpheus for hybrid DB/LA workloads over relational data.

==> figures/tarns_vec.tex <==
\begin{figure*}[t]
\begin{tabular}{|l|r c l|c|}
\hline
\textbf{Name} & \multicolumn{3}{|l|}{\textbf{Translation}} & \textbf{Einsum} \\ \hline
Addition &\translate{$V_1 + V_2$} &=& \translate{$V_1$} !+!  \translate{$V_2$}& - \\ \hline 
Scal-Vec. Mul.&\translate{$a \cdot V$} &=& \translate{$a$} !*! \translate{$V$}& !,i->i! \\ \hline 
Hadamard Prod.&\translate{$V_1 \circ V_2$} &=& !sum(x in! \translate{$V_1$} !) { x.key->x.val*!\translate{$V_2$}!(x.key) }! & !i,i->i! \\ \hline
Dot Prod.&\translate{$V_1 \cdot V_2$} &=& !sum(x in! \translate{$V_1$} !) x.val * !\translate{$V_2$}!(x.key)!& !i,i->! \\ \hline 
Summation&\translate{$\sum_{a\in V}a$} &=& !sum(x in! \translate{$V$} !) x.val!&!i->! \\ \hline 
\end{tabular}
\vspace{-0.3cm}
\caption{Translation of vector operations to \lang.}
\label{fig:vec_ndql}
\vspace{-0.3cm}
\end{figure*}

==> figures/types_denot_semantics.tex <==
\begin{figure*}[t]
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{|c|}
\hline
% \begin{tabular}{c c}
\begin{tabular}{l c l}
\dsnoctx{\code{S}} & \myeq & ($S$, $+$, $0$) \\
\dsnoctx{\code{<a1:T1, ..., an:Tn>}} & \myeq  &\dsnoctx{\code{T1}} $\times$ ... $\times$ \dsnoctx{\code{Tn}} \\
\dsnoctx{\code{\{T1 -> T2\}}} & \myeq  & $\sumplus\limits_{a \in |T1|}$\dsnoctx{\code{T2}}\\
\dsnoctx{\code{T1} $\otimes_S$ \code{T2}} & \myeq  & \dsnoctx{\code{T1}} $\otimes_S$ \dsnoctx{\code{T2}} \\
\end{tabular}\\
% &
% \begin{tabular}{l c l}
% \dsnoctx{\code{S}} & \myeq  & ($S$, $+$, $0$) \\
% \dsnoctx{\code{<a1:T1, ..., an:Tn>}} & \myeq  &\dsnoctx{\code{T1}} $\times$ ... $\times$ \dsnoctx{\code{Tn}} \\
% \dsnoctx{\code{\{T1 -> T2\}}} & \myeq  & $\sumplus\limits_{a \in |T1|}$\dsnoctx{\code{T2}}\\
% \dsnoctx{\code{T1} $\otimes_S$ \code{T2}} & \myeq  & \dsnoctx{\code{T1}} $\otimes_S$ \dsnoctx{\code{T2}} \\
% \end{tabular}
% \end{tabular}\\
\hline
\end{tabular}
\vspace{-0.4cm}
\caption{Denotational Semantics for types of \lang.}
\vspace{-0.4cm}
\label{fig:types_denot_sem}
\end{figure*}
